Evolution of the Archean Atmosphere

Archean atmospheric evolution is the transition from an abiological atmosphere, to an atmosphere for which the composition and therefore climate is highly altered by life. We review the key processes and transitions in this evolution.

==> unusedtext.tex <==
\section{On constraints: proxy, theory, and all the models}
% THe point that I want to make here is that almost anything quantatitve has a model component to it. 
% I'm not hugely happy wit the text as is. 
\emph{``Oh, you study past climate! Do you use ice cores?''}

For the middle and upper Pleistocene, palaeoclimatologists may study actual bubbles of past atmosphere, frozen in ice, and determining atmospheric composition is simply a measurement problem (albeit a delicate one). Deeper in time, no such luxury exists, and our data-based controls on the atmospheric composition decrease exponentially with age. Old rocks are few, and altered. 

Empirical constraints on the ancient atmosphere come from proxy measurements. That is, \emph{something else entirely is measured}, then a \emph{model} is used to translate the measured quantity into a parameter of interest. There are


A value is quoted in the abstract of the paper, cited widely, and the actual measurement and model are typically forgotten. There are two general categories criticism. First, that the measurement may not be as seems: later alteration of rocks  may have altered the measured quantity. With the vastness of time since the Archean, this is a scourge. Second, and most insidious, are the models. Chains of assumptions need be made about what processes occurred and at what rate, requiring numerous arbitrary assumptions, which may affect both accuracy and precision. 

The radical exception to the general paucity of evidence is for oxygen and ozone. We know of a Great Oxidation because of change to the atmosphere large enough to transition the surface from reducing to oxidising conditions, changing so much of the chemistry, and preserving abundant records. Yet this is in the context of a change in oxygen mixing ratios of perhaps six orders of magnitude over the whole Archean, and at least two orders of magnitude at Great Oxidation itself. No other species has changed so much, nor left so much record. 

Constraints on individual species are summarized in Section REF. 

Necessarily, therefore, the development of theory plays a great role in developing understanding of Archean atmospheric evolution. While time ravages rocks, the laws physics and chemistry that govern Earth do not change. A wide ranging view of Earth-system processes, from biogeochemisty to climate physics, is brought to use. Two principle factors differentiate this from the modern Earth system. First, the abundance of time, for small imbalances in geochemical fluxes come to have a dominant effect of the timescale of a billion years. Second is diversity of process: if anything is possible, it probably happened at some point in the past. 

The point of this section is to say that the boundary between data and models is not that big, and one should always interogate what the models actually mean. [and after writing, I'm not hugely happy with it]

